Black-Box Safety Validation of Autonomous Systems: A Multi-Fidelity Reinforcement Learning Approach

The increasing use of autonomous and semi-autonomous agents in society has made it crucial to validate their safety. However, the complex scenarios in which they are used may make formal verification impossible. To address this challenge, simulation-based safety validation is employed to test the complex system. Recent approaches using reinforcement learning are prone to excessive exploitation of known failures and a lack of coverage in the space of failures. To address this limitation, a type of Markov decision process called the "knowledge MDP" has been defined. This approach takes into account both the learned model and its metadata, such as sample counts, in estimating the system's knowledge through the "knows what it knows" framework. A novel algorithm that extends bidirectional learning to multiple fidelities of simulators has been developed to solve the safety validation problem. The effectiveness of this approach is demonstrated through a case study in which an adversary is trained to intercept a test model in a grid-world environment. Monte Carlo trials compare the sample efficiency of the proposed algorithm to learning with a single-fidelity simulator and show the importance of incorporating knowledge about learned models into the decision-making process.

==> algs.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}
%    \SetAlgoLined
\caption{KWIK-AST}\label{alg:kwik_ast}
\SetKw{Input}{input:}
\SetKw{Output}{output:}
\SetKw{Initialize}{initialize:}
%\SetKwFunction{Search}{search}
\SetKwProg{Proc}{Procedure}{}{}

\Input{$s$, $\Sigma$, $\mathcal{M}$, $R_{max}$, $R_{inc}$, $P$, $\langle \epsilon, \delta \rangle$}

\Initialize{ $\hat{R}$ , $\hat{T}$, $\mathcal{K}_R$, $\mathcal{K}_T$, $Q$}

\Proc{evaluateSample($s$)}
{
$f \leftarrow \{\}$

$is\_converged = true$

\While{$\neg terminal(s)$}
{
    $a \leftarrow \{ P.getPolicy(s), \mathcal{M}.getPolicy(s)\}$
    
    $s',r \sim T_\Sigma(s'|s,a)$
    
    $f \leftarrow f \cup \langle s, a, s' \rangle$
    
    \If  {$\mathcal{K}_T(s)$ or $\mathcal{K}_R(s) == \perp $}
    {
        Update $\hat{T}(s,a,s')$, $\hat{R}(s,a,s')$
        
        Update $\mathcal{K}_T(s)$, $\mathcal{K}_R(s)$
        
        $Q \leftarrow P.train(\hat{T},\hat{R},Q)$
        
        $is\_converged = false$
    }
    $s \leftarrow s'$
}
\If {is\_converged}
{
    $marginalUpdate(f)$
    
     $Q \leftarrow P.train(\hat{T},\hat{R},Q)$
}
\If {$isFailure(f)$}
{
\Return $f$
}\Else
{
\Return $\{\}$
}
}

\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}
%    \SetAlgoLined
\caption{search}\label{alg:kwik_ast}
\SetKw{Input}{input:}
\Input{$s$,$n$}

$\mathcal{\hat{F}} \leftarrow \{\}$

\For {$i = 1, ..., n$}
{
    reinitialize $\Sigma$
    
    $\mathcal{\hat{F}} \leftarrow \mathcal{\hat{F}} \cup evaluateSample(s)$    
}

\For {$f \in \mathcal{\hat{F}}$}
{
    \If {$\neg isPlausible(f,D)$}
    {
        $\mathcal{\hat{F}} \leftarrow \mathcal{\hat{F}} \setminus f$
    }
}
    
\Return $\mathcal{\hat{F}}$


\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
%    \SetAlgoLined
\caption{marginalUpdate}\label{alg:kwik_ast}
\SetKw{Input}{input:}

\Input{$f$}
{
$m_{max} \leftarrow 0$

$transition \leftarrow \langle \rangle$

\For {$\langle s, a, s' \rangle \in f$}
{
    $m = Q^*(s,a) - Q^{**}(s,a)$
    
    %\arg\max_{a' \in (A \setminus a)}  \sum_{s''} T(s,a',s'')(R(s,a',s'',\mathcal{K}) + \gamma Q(s'',a'))$
    
    \If{$m > m_{max}$}
    {
        $m_{max} \leftarrow m$
        
        $transition \leftarrow \langle s, a, s' \rangle$
    }
}

$R(transition) \leftarrow R(transition) - R_{inc}$
}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{MF-KWIK-AST}

\begin{algorithm}
%    \SetAlgoLined
\caption{MF-KWIK-AST}\label{alg:kwik_ast}
\SetKw{Input}{input:}
\SetKw{Output}{output:}
\SetKw{Initialize}{initialize:}
%\SetKwFunction{Search}{search}
\SetKwProg{Proc}{Procedure}{}{}

\Input{$s$, $\langle \Sigma, \beta, \rho \rangle$, $\mathcal{M}$, $R_{max}$, $R_{inc}$, $P$, $\langle \epsilon, \delta, m_known, m_unknown \rangle$}

\Initialize{ $\hat{R}$ , $\hat{T}$, $\mathcal{K}_R$, $\mathcal{K}_T$, $Q_d$}
\Initialize{ $change_d = false, Q_0 = \dfrac{R_{max}}{1-\gamma}, d = 1, m_k,m_u = 0$}

\Proc{evaluateSample($s$)}
{
$f \leftarrow \{\}$

$is\_converged = true$

\While{$\neg terminal(s)$}
{
    $a \leftarrow \{ P.getPolicy(s), \mathcal{M}.getPolicy(s)\}$
    
    $s',r \sim T_\Sigma(s'|s,a)$
    
    $f \leftarrow f \cup \langle s, a, s' \rangle$
    
    \If{$d>1$ and $change_d$ and ($K_{T,d-1}(\rho_{d-1}^{-1}(s),a_{KWIK})$ or $K_{R,d-1}(\rho_{d-1}^{-1}(s),a_{KWIK}) = \perp$}
    {
        $Q_{d-1} \leftarrow plan(d)$
        
        $m_k \leftarrow 0$, $m_u \leftarrow 0$
        
        $ d \leftarrow d-1$
        
        $change_{d-1} = false$
    }
    \Else
    {
    \If  {$\mathcal{K}_T(s)$ or $\mathcal{K}_R(s) == \perp $}
    {
        Update $\hat{T}(s,a,s')$, $\hat{R}(s,a,s')$
        
        Update $\mathcal{K}_T(s)$, $\mathcal{K}_R(s)$
        
        \If {$\mathcal{K}_T(s)$ or $\mathcal{K}_R(s) becomes known $}
        {   
            $Q_{d} \leftarrow plan(d)$
            $m_k \leftarrow m_k + 1$, $m_u \leftarrow 0$
        }
        \Else
        {
        $m_k \leftarrow 0$, $m_u \leftarrow m_u + 1$
        }
        $is\_converged = false$
    }
    \Else
    {
        $m_k \leftarrow m_k + 1$, $m_u \leftarrow 0$
    }
    $s \leftarrow s'$
    }
    
    \If{$d < D$ and $m_k >= m_known$}
    {
        $change_d = false$
        
        $d \leftarrow d + 1$
        
        $Q_{d} \leftarrow plan(d)$
        
        $m_k \leftarrow 0$, $m_u \leftarrow 0$
    }
}
\If {is\_converged}
{
    $marginalUpdate(f)$
    
     $Q \leftarrow P.train(\hat{T},\hat{R},Q)$
}
\If {$isFailure(f)$}
{
\Return $f$
}\Else
{
\Return $\{\}$
}

\Proc{plan(d)}
{
\For{ all $\langle s, a \rangle$}
{
    Find $d' >= d, s.t. K_{T,d'} is known and T_d(s,a,:) \leftarrow T_{d'}(s,a,:)$ 
    Find $d' >= d, s.t. K_{R,d'} is known and T_d(s,a,:) \leftarrow R_{d'}(s,a,:)$ 
}

$Q \leftarrow P.train(\hat{T},\hat{R},Q, Q_{d-1}+\beta_{d-1})$
}

}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{KWIK-AST}

What do we want to answer here? 

Introduce the KWIK Rmax algorithm
    Discuss details of algorithm / implementation
    Discuss how optimisim iFoU helps exploration
    Introduce marginal update to prevent early convergence (when we move on to MF algorithm, this should cause search in higher fidelities to be delayed


Refine algorithms to take R,T


\RestyleAlgo{ruled}
\begin{algorithm}
%    \SetAlgoLined
\caption{KWIK-AST}\label{alg:kwik_ast}
\SetKw{Input}{input:}
\SetKw{Output}{output:}
\SetKw{Initialize}{initialize:}
%\SetKwFunction{Search}{search}
\SetKwProg{Proc}{Procedure}{}{}

\Input{$s$, $\Sigma$, $\mathcal{M}$, $R_{max}$, $R_{inc}$, $P$, $\langle \epsilon, \delta \rangle$}

\Initialize{ $\mathcal{K}$, $Q$}

\Proc{evaluateSample($s$)}
{
$f \leftarrow \{\}$

$is\_converged = true$

\While{$\neg terminal(s)$}
{
    $a \leftarrow \{ P.getPolicy(s), \mathcal{M}.getPolicy(s)\}$
    
    $s',r \sim T_\Sigma(s'|s,a)$
    
    $f \leftarrow f \cup \langle s, a, s' \rangle$
    
    \If  {$\mathcal{K}_T$, $\mathcal{K}_R ==$ $\perp $}
    {
        Update $\mathcal{K}$
        
        $Q \leftarrow P.train(\mathcal{K}.\hat{T}$, $\mathcal{K}.\hat{R}$, $Q)$
        
        $is\_converged = false$
    }
    $s \leftarrow s'$
}
\If {is\_converged}
{
    $marginalUpdate(f)$
    
     $Q \leftarrow P.train(\mathcal{K}.\hat{T}$, $\mathcal{K}.\hat{R}$, $Q)$
}
\If {$isFailure(f)$}
{
\Return $f$
}
}

\end{algorithm}

==> formatting_guidelines.tex <==
\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as Ò3.5-inch disk driveÓ.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ÒWb/m2Ó or Òwebers per square meterÓ, not Òwebers/m2Ó.  Spell out units when they appear in text: Ò. . . a few henriesÓ, not Ò. . . a few HÓ.
\item Use a zero before decimal points: Ò0.25Ó, not Ò.25Ó. Use Òcm3Ó, not ÒccÓ. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use Ò(1)Ó, not ÒEq. (1)Ó or Òequation (1)Ó, except at the beginning of a sentence: ÒEquation (1) is . . .Ó

\subsection{Some Common Mistakes}
\begin{itemize}


\item The word ÒdataÓ is plural, not singular.
\item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ÒoÓ.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ÒinsetÓ, not an ÒinsertÓ. The word alternatively is preferred to the word ÒalternatelyÓ (unless you really mean something that alternates).
\item Do not use the word ÒessentiallyÓ to mean ÒapproximatelyÓ or ÒeffectivelyÓ.
\item In your paper title, if the words Òthat usesÓ can accurately replace the word ÒusingÓ, capitalize the ÒuÓ; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ÒaffectÓ and ÒeffectÓ, ÒcomplementÓ and ÒcomplimentÓ, ÒdiscreetÓ and ÒdiscreteÓ, ÒprincipalÓ and ÒprincipleÓ.
\item Do not confuse ÒimplyÓ and ÒinferÓ.
\item The prefix ÒnonÓ is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ÒetÓ in the Latin abbreviation Òet al.Ó.
\item The abbreviation Òi.e.Ó means Òthat isÓ, and the abbreviation Òe.g.Ó means Òfor exampleÓ.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named ÒHeading 1Ó, ÒHeading 2Ó, ÒHeading 3Ó, and ÒHeading 4Ó are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ÒFig. 1Ó, even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó
